More Than Mimicking Reviewers: Evaluating LLMs for Pre-Submission Peer Review

Peer-review feedback often arrives too late for authors to make meaningful revisions. We study an author-facing LLM system that moves part of this stress test before submission: it generates a broad pool of atomic concerns and compresses them into a short report. We evaluate agreement with historical reviews and, separately, the possible validity of concerns they omit. From 10,000 ICLR 2026 submissions, we use 3,398 manuscripts with accessible versions that predate review. On a ten-paper diagnostic, independent sampling covers 44.9% of historical issues; deduplication and refill reaches 78.7% strict and 84.9% seriousness-weighted coverage, at 3.6$\times$ more requests and 5.2$\times$ more tokens. A hidden Top-32 Oracle preserves the full 79.3% weighted coverage of a 256-candidate pool, but paper-only selectors retain only 40--44%. LLM review therefore provides broad coverage with a large candidate pool but compresses poorly; ablations identify representative selection and matcher sensitivity as the main sources of this gap.

==> sections/06_acceptance_judging.tex <==
\section{Do human reviews improve acceptance judging?}
\label{sec:acceptance-judging}

We separately test whether additional evidence helps an LLM judge forecast the
conference outcome. This exploratory diagnostic uses 15 disjoint training
papers selected as five Oral, five Poster, and five Reject; Oral and Poster are
merged at evaluation, giving 10 Accept and five Reject papers. Withdrawn is
excluded. Every judge receives the title, the same paper-only
\texttt{spr\_medium} representation, and a leave-cohort-out training prior.
The four judges are DeepSeek V4 Flash, Kimi-K3, Inkling NVFP4, and GPT-5.6 Sol
High, all run at temperature zero.

We compare two information conditions. \emph{Paper only} excludes reviews,
scores, rebuttals, discussion, meta-review, venue, and decision. \emph{Paper +
reviews} adds the actual anonymous summaries, strengths, weaknesses, questions,
and limitations, but removes ratings, confidence, identities, replies,
meta-review, and decision. Fourteen papers have three or four reports; one
Reject paper has none and receives an empty list. Because current review notes
may contain post-rebuttal edits, this is an information upper bound rather than
a feasible paper-only forecast.

\input{tables/acceptance_judging}

Figure~\ref{fig:acceptance-judging} exposes a strong judge--context
interaction. No paper-only judge exceeds the 0.667 majority-Accept accuracy;
paper-only AUROC ranges from 0.460 to 0.640. Adding review prose raises Kimi
from 0.333/0.460 to 0.733/0.820 accuracy/AUROC and Sol from 0.467/0.520 to
0.800/0.920. It instead lowers DeepSeek accuracy from 0.467 to 0.400 and
Inkling accuracy from 0.667 to 0.467. Inkling's AUROC nevertheless rises from
0.640 to 0.700, indicating a threshold or calibration shift rather than a pure
loss of ranking information. Sol with reviews also has the best NLL (0.528)
and Brier score (0.178).

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/acceptance_judging_context.pdf}
  \caption{The effect of adding sanitized human-review prose depends on the
  judge. Lines connect the same model across conditions. The dashed references
  are majority-Accept accuracy (0.667) in (a) and chance AUROC (0.500) in (b)
  on this 10:5 binary cohort.}
  \label{fig:acceptance-judging}
\end{figure}

This is not a causal or confirmatory comparison. It uses only 15 training
papers; the non-Sol paper-only extension ran through isolated frozen inputs
after the Sol labels had been opened; and the paper-only responses were
originally four-way forecasts later collapsed to Accept/Reject, whereas the
review-informed prompt requested binary probabilities directly. The safe
conclusion is therefore narrower: human review text is highly predictive for
some LLM judges, but merely providing it does not reliably improve every judge.


==> sections/06_limitations.tex <==
\section{Limitations and responsible use}

Although broad generation recovers much of the historical issue weight and our
ablations isolate clear compression and evaluation bottlenecks, the evidence is
not yet sufficient for a generalization claim: most results come from ten
training papers, the mixture pilot uses five validation papers, and the
680-paper test remains unopened. The remaining errors can be addressed
separately. Generation comparisons still couple some policy and serving
choices; historical reviews and their atomization provide incomplete targets;
the Sol matcher determines most reported edges; and AI-only examples and
Top-32 rankings await a completed expert audit. The DeepSeek scale collapse and
Sol selection skew may also be deployment-specific rather than model-wide
effects. Accordingly, an author-facing system should expose evidence and
uncertainty, separate reviewer likelihood from independent validity, and be
positioned as revision support rather than acceptance prediction, validation
of a research idea, or a replacement for human review.

